Which are Better Conditioned Meshes Adaptive, Uniform, Locally Refined or Localised

Adaptive, locally refined and locally adjusted meshes are preferred over uniform meshes for capturing singular or localised solutions. Roughly speaking, for a given degree of freedom a solution associated with adaptive, locally refined and locally adjusted meshes is more accurate than the solution given by uniform meshes. In this work, we answer the question which meshes are better conditioned. We found, for approximately same degree of freedom (same size of matrix), it is easier to solve a system of equations associated with an adaptive mesh.

==> Makefile <==
# Generic make file for LaTeX: requires GNU make
#
# This makefile provides four targets: dvi, ps, pdf and clean.
# The default is "pdf".
# To make a dvi file, type "make dvi"
# To make a ps file, type "make ps".
# To make a pdf file, type "make pdf" or simply "make".
# To remove all files generated by make, type "make clean".
#
# Rouben Rostmaian
# September 2002

TEXFILE =   article.tex
#TEXFILE	= slides.texTPFA_diagonal_perm_variable.tex

.PHONY: dvi ps pdf clean

pdf:	$(TEXFILE:.tex=.pdf)
ps:	$(TEXFILE:.tex=.ps)
dvi:	$(TEXFILE:.tex=.dvi)

%.dvi: %.tex
	( \
	\latex $<; \
	while \grep -q "Rerun to get cross-references right." $(<:.tex=.log); \
	do \
		\latex $<; \
	done \
	)

%.ps: %.dvi
	\dvips -q -t a4 $<

%.pdf: %.ps
	\ps2pdf -dPDFSETTINGS=/prepress $<

clean:
	@\rm -f \
	$(TEXFILE:.tex=.aux) \
	$(TEXFILE:.tex=.log) \
	$(TEXFILE:.tex=.out) \
	$(TEXFILE:.tex=.dvi) \
	$(TEXFILE:.tex=.ps)

